Binary Optimal Control Of Single-Flux-Quantum Pulse Sequences

We introduce a binary, relaxed gradient, trust-region method for optimizing pulse sequences for single flux quanta (SFQ) control of a quantum computer. The pulse sequences are optimized with the goal of realizing unitary gate transformations. Each pulse has a fixed amplitude and duration. We model this process as an binary optimal control problem, constrained by Schr\"{o}dinger's equation, where the binary variables indicate whether each pulse is on or off. We introduce a first-order trust-region method, which takes advantage of a relaxed gradient to determine an optimal pulse sequence that minimizes the gate infidelity, while also suppressing leakage to higher energy levels. The proposed algorithm has a computational complexity of ${\cal O}(p\log(p)$, where $p$ is the number of pulses in the sequence. We present numerical results for the H and X gates, where the optimized pulse sequences give gate fidelity's better than $99.9\%$, in $\approx 25$ trust-region iterations.

==> Makefile <==
SOURCE = article
TEXFILES = *.tex
BIBFILES = *.bib
TIKZFILES = 
PDFFILES = 
COVER_FILE = 
SUPP_FILES = article_supp

all: $(SOURCE).pdf 

$(SOURCE).pdf: $(TEXFILES) $(BIBFILES) $(PDFFILES) $(TIKZFILES)
	pdflatex --shell-escape $(SOURCE).tex
	pdflatex $(SOURCE)_supp.tex
	pdflatex $(SOURCE)_supp.tex
	bibtex $(SOURCE)
	pdflatex --shell-escape $(SOURCE).tex
	pdflatex --shell-escape $(SOURCE).tex
#	dvipdf $(SOURCE).dvi

supp: $(SUPP_FILES).pdf
	pdflatex --shell-escape $(SUPP_FILES).tex
	bibtex $(SUPP_FILES)
	pdflatex --shell-escape $(SUPP_FILES).tex

cover: $(COVER_FILE).pdf
	pdflatex --shell-escape $(COVER_FILE).tex

ANL: $(TEXFILES) $(BIBFILES) $(PDFFILES) $(TIKZFILES)
	pdflatex --shell-escape P9167-0319.tex
	bibtex P9167-0319
	pdflatex --shell-escape P9167-0319.tex
	pdflatex --shell-escape P9167-0319.tex

.SUFFIXES: .fig .pdf

.fig.pdf:
	fig2dev -L pdf -p dummy $< $@

#$(preprint).pdf: $(TEXFILES) 
#  pdflatex $(preprint).tex

#$(response).pdf: $(TEXFILES) 
#  pdflatex $(response).tex

view: $(SOURCE).pdf
	open $(SOURCE).pdf
clean:
	-rm -f  *.thm *.toc *.log *.aux *.auxlock *.bbl *.blg *.out \
	$(SOURCE).pdf *.backup *.tex~ *.log MIPDFO.pdf


